Towards a Game-Theoretic Security Analysis of Off-Chain Protocols

Off-chain protocols constitute one of the most promising approaches to solve the inherent scalability issue of blockchain technologies. The core idea is to let parties transact on-chain only once to establish a channel between them, leveraging later on the resulting channel paths to perform arbitrarily many peer-to-peer transactions off-chain. While significant progress has been made in terms of proof techniques for off-chain protocols, existing approaches do not capture the game-theoretic incentives at the core of their design, which led to overlooking significant attack vectors like the Wormhole attack in the past. In this work we take a first step towards a principled game-theoretic security analysis of off-chain protocols by introducing the first game-theoretic model that is expressive enough to reason about their security. We advocate the use of Extensive Form Games (EFGs) and introduce two instances of EFGs to capture security properties of the closing and the routing of the Lightning Network. Specifically, we model the closing protocol, which relies on punishment mechanisms to disincentivize parties to upload old channel states on-chain. Moreover, we model the routing protocol, thereby formally characterizing the Wormhole attack, a vulnerability that undermines the fee-based incentive mechanism underlying the Lightning Network.

==> cleveref/README <==
cleveref, a LaTeX package for intelligent cross-referencing
Copyright (C) 2007--2018  Toby Cubitt

Files:
cleveref.ins  Batch file, run through LaTeX
cleveref.dtx  Docstrip archive, run through LaTeX
cleveref.sty  LaTeX package, generated by cleveref.ins from cleveref.dtx
cleveref.dvi  Package documentation, generated from cleveref.dtx
cleveref.pdf  Package documentation; can also be generated from cleveref.dtx
README        This file

E-mail:   toby-cleveref@dr-qubit.org
Address:  Department of Computer Science, UCL, United Kingdom

This material is subject to the LaTeX Project Public License. See
http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the
details of that license.


Description:
------------
The cleveref package enhances LaTeX's cross-referencing features, allowing the
format of cross-references to be determined automatically according to the
"type" of cross-reference (equation, section, etc.) and the context in which
the cross-reference is used. The formatting for each cross-reference type can
be fully customised in the preamble of your document. In addition, cleveref
can type-set cross-references to lists of multiple labels, automatically
formatting them according to their types, sorting them, and compressing
sequences of numerically consecutive labels. Again, the multiple-reference
formatting is fully customisable. Though a number of other packages provide
similar features, all have certain deficiencies which cleveref attempts to
overcome.

Using cleveref is easy. Basically, wherever you would previously have used
\ref, you can use \cref instead. (Except at the beginning of a sentence, where
you should use \Cref.)  You no longer need to put the name of the thing you're
referencing in front of the \cref command, because cleveref will sort that out
for you: i.e. use "\cref{eq1}" instead of "eq.~(\ref{eq1})". If you want to
refer to a range of labels, use the \crefrange command: "\crefrange{eq1}{eq5}"
produces "eqs.~(1) to~(5)". Finally, if you want to refer to multiple things
at once, you can now combine them all into one cross-reference and leave
cleveref to sort it out: e.g. "\cref{eq2,eq1,eq3,eq5,thm2,def1}" produces:
"eqs.~(1) to~(3) and~(5), theorem~5, and definition~1".

Cleveref has various other useful features. For details, see the package
documentation.


==> includes/acknowledgements.tex <==
\section*{Acknowledgements}
This research was supported by the ERC Grant BROWSEC 771527, the ERC Grant ARTIST 101002685, the Austrian Science Fund FWF projects W1255-N23, and PROFET P31621, the Austrian Research Promotion Agency FFG through the Bridge-1 project PR4DLT (13808694) and the COMET K1 SBA, the Amazon Research Award 2020 FOREST, and the SecInt Doctoral College funded by TU Wien.

%This work has been supported by the European Research Council (ERC) under the Horizon 2020 research (grant 771527-BROWSEC); by the Austrian Science Fund (FWF) through the projects PROFET (grant P31621) and the project W1255- N23; by the Austrian Research Promotion Agency (FFG) through the Bridge-1 project PR4DLT (grant 13808694) and the COMET K1 SBA; by the Vienna Business Agency through the project Vienna Cybersecurity and Privacy Re- search Center (VISP).

%This research was supported by the  XXX, ERC Consolidator Grant ARTIST 101002685, the Austrian FWF project W1255-N23, the Amazon Research Award 2020 FORST, and the SecInt Doctoral College funded by TU Wien."

==> includes/appendices/subgames.tex <==
\subsection{Subgames of the Closing Game} \label{app:subgames}
In the following all the subgames needed for the closing game $G_c(A)$ are defined.

The subgames $S_1$ and $S_2$ in \Cref{tbl:S1} and \Cref{tbl:S2} cover the case where a channel update is proposed by $A$, although $A$ has already signed an honest collaborative closing attempt. In $S_1$ the update is from channel state $(a,b)$ to $(a+p_A,b-p_A)$, whereas in $S_2$ the suggested update is $(a-p_B, b+p_B)$. 




\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{olive}$B$};
		
		%B block top
		\node (20) at (1,-2.25) {\color{teal} $A$};
		\node (2) at (1.75,-2.75) {\color{teal}$A$} ; 
		\node (3) at (-1.,-0.25) {\color{teal}$A$};
		\node (21) at (-1,0.5) {$(\alpha,\alpha-\epsilon)$};
		\node (24) at (-0.15,-1.25) {$(\alpha,\alpha)$};
		
		%A block middle
		\node (22) at (-2.,-3.25) {$(b-f+\alpha,-b)$};
		\node (23) at (-3.5,-2.75) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
				
		%A block left
		\node (8) at (-3.25,-2) {$(-a,-b)$};
		\node (9) at (-1.75,-2.) {$(\alpha-\epsilon,\alpha)$};
		\node (10) at (-2.25,-0.5) {\color{olive}$B$};
		
		%A block right
		\node (5) at (1.75,-5.75) {\color{olive}$B$};
		\node (6) at (-1,-4) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (7) at (1,-4.25) {\color{olive}$B$};
		
		%B block middle
		\node (11) at (-1.25,-5.5) {$(-a{\color{red}-p_A}+\rho,a{\color{red}+p_A}-f+\rho+\alpha)$};
		\node (12) at (-3.25,-5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		%B block left
		\node (13) at (-5,-0.75) {$(-a,a-f+\alpha)$};
		\node (14) at (-4.35,-1.25) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
		
		%B block right
		\node (15) at (1.75,-8.25) {\color{teal}$A$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}-p_A}+\rho,-b{\color{red}+p_A}+\rho)$};
		\node (4) at (-3.75,-6.75) {$({\color{red}-p_A}+\rho+\alpha,{\color{red}p_A}+\rho+\alpha)$};
		
		%A block bottom
		\node (18) at (-3,-9) {$(b{\color{red}-p_A}-f+\rho+\alpha,-b{\color{red}+p_A}+\rho)$};
		\node (19) at (-0.5,-9.5) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		{\color{olive}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.5] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);
		\path (1) edge node [left] {\tiny $S$} (24); }
		
		{\color{teal}
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);

		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{olive}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);
		\path (5) edge node [above] {\tiny $S$}  (4);}
		
		{\color{teal}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S_{1}$ with Update $(a,b)\mapsto (a+p_A,b-p_A)$.}
	\label{tbl:S1}
\end{figure}






\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{olive}$B$};
		
		%B block top
		\node (20) at (1,-2.25) {\color{teal} $A$};
		\node (2) at (1.75,-2.75) {\color{teal}$A$} ; 
		\node (3) at (-1.,-0.25) {\color{teal}$A$};
		\node (21) at (-1,0.5) {$(\alpha,\alpha-\epsilon)$};
		\node (24) at (-0.15,-1.25) {$(\alpha,\alpha)$};
		
		%A block middle
		\node (22) at (-2.,-3.25) {$(b-f+\alpha,-b)$};
		\node (23) at (-3.5,-2.75) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
				
		%A block left
		\node (8) at (-3.25,-2) {$(-a,-b)$};
		\node (9) at (-1.75,-2.) {$(\alpha-\epsilon,\alpha)$};
		\node (10) at (-2.25,-0.5) {\color{olive}$B$};
		
		%A block right
		\node (5) at (1.75,-5.75) {\color{olive}$B$};
		\node (6) at (-1,-4) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (7) at (1,-4.25) {\color{olive}$B$};
		
		%B block middle
		\node (11) at (-1.25,-5.5) {$(-a{\color{red}+p_B}+\rho,a{\color{red}-p_B}-f+\rho+\alpha)$};
		\node (12) at (-3.25,-5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		%B block left
		\node (13) at (-5,-0.75) {$(-a,a-f+\alpha)$};
		\node (14) at (-4.35,-1.25) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
		
		%B block right
		\node (15) at (1.75,-8.25) {\color{teal}$A$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}+p_B}+\rho,-b{\color{red}-p_B}+\rho)$};
		\node (4) at (-3.75,-6.75) {$({\color{red}p_B}+\rho+\alpha,{\color{red}-p_B}+\rho+\alpha)$};
		
		%A block bottom
		\node (18) at (-3,-9) {$(b{\color{red}+p_B}-f+\rho+\alpha,-b{\color{red}-p_B}+\rho)$};
		\node (19) at (-0.5,-9.5) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		{\color{olive}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.5] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);
		\path (1) edge node [left] {\tiny $S$} (24); }
		
		{\color{teal}
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);

		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{olive}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);
		\path (5) edge node [above] {\tiny $S$}  (4);}
		
		{\color{teal}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S_{2}$ with Update $(a,b)\mapsto (a-p_B,b+p_B)$.}
	\label{tbl:S2}
\end{figure}






The subgames $S_1'$ and $S_2'$ in \Cref{tbl:S1p} and \Cref{tbl:S2p} are very similar to $S_1$ and $S_2$. They only differ in the fact, that the existing partially signed collaborative closing attempt was dishonest. That means, $A$ proposed an unfair split, increasing her outcome by value $c>0$.



\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{olive}$B$};
		
		%B block top
		\node (20) at (1,-2.25) {\color{teal} $A$};
		\node (2) at (1.75,-2.75) {\color{teal}$A$} ; 
		\node (3) at (-1.,-0.25) {\color{teal}$A$};
		\node (21) at (-1,0.5) {$(\alpha,\alpha-\epsilon)$};
		\node (24) at (-0.15,-1.25) {$({\color{red}c}+\alpha,{\color{red}-c}+\alpha)$};
		
		%A block middle
		\node (22) at (-2.,-3.25) {$(b-f+\alpha,-b)$};
		\node (23) at (-3.5,-2.75) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
				
		%A block left
		\node (8) at (-3.25,-2) {$(-a,-b)$};
		\node (9) at (-1.75,-2.) {$(\alpha-\epsilon,\alpha)$};
		\node (10) at (-2.25,-0.5) {\color{olive}$B$};
		
		%A block right
		\node (5) at (1.75,-5.75) {\color{olive}$B$};
		\node (6) at (-1,-4) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (7) at (1,-4.25) {\color{olive}$B$};
		
		%B block middle
		\node (11) at (-1.25,-5.5) {$(-a{\color{red}-p_A}+\rho,a{\color{red}+p_A}-f+\rho+\alpha)$};
		\node (12) at (-3.25,-5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		%B block left
		\node (13) at (-5,-0.75) {$(-a,a-f+\alpha)$};
		\node (14) at (-4.35,-1.25) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
		
		%B block right
		\node (15) at (1.75,-8.25) {\color{teal}$A$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}-p_A}+\rho,-b{\color{red}+p_A}+\rho)$};
		\node (4) at (-3.75,-6.75) {$({\color{red}c-p_A}+\rho+\alpha,{\color{red}-c+p_A}+\rho+\alpha)$};
		
		%A block bottom
		\node (18) at (-3,-9) {$(b{\color{red}-p_A}-f+\rho+\alpha,-b{\color{red}+p_A}+\rho)$};
		\node (19) at (-0.5,-9.5) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		{\color{olive}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.5] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);
		\path (1) edge node [left] {\tiny $S$} (24); }
		
		{\color{teal}
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);

		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{olive}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);
		\path (5) edge node [above] {\tiny $S$}  (4);}
		
		{\color{teal}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S'_{1}$ with Update $(a,b)\mapsto (a+p_A,b-p_A)$.}
	\label{tbl:S1p}
\end{figure}




\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{olive}$B$};
		
		%B block top
		\node (20) at (1,-2.25) {\color{teal} $A$};
		\node (2) at (1.75,-2.75) {\color{teal}$A$} ; 
		\node (3) at (-1.,-0.25) {\color{teal}$A$};
		\node (21) at (-1,0.5) {$(\alpha,\alpha-\epsilon)$};
		\node (24) at (-0.15,-1.25) {$({\color{red}c}+\alpha,{\color{red}-c}+\alpha)$};
		
		%A block middle
		\node (22) at (-2.,-3.25) {$(b-f+\alpha,-b)$};
		\node (23) at (-3.5,-2.75) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
				
		%A block left
		\node (8) at (-3.25,-2) {$(-a,-b)$};
		\node (9) at (-1.75,-2.) {$(\alpha-\epsilon,\alpha)$};
		\node (10) at (-2.25,-0.5) {\color{olive}$B$};
		
		%A block right
		\node (5) at (1.75,-5.75) {\color{olive}$B$};
		\node (6) at (-1,-4) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (7) at (1,-4.25) {\color{olive}$B$};
		
		%B block middle
		\node (11) at (-1.25,-5.5) {$(-a{\color{red}+p_B}+\rho,a{\color{red}-p_B}-f+\rho+\alpha)$};
		\node (12) at (-3.25,-5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		%B block left
		\node (13) at (-5,-0.75) {$(-a,a-f+\alpha)$};
		\node (14) at (-4.35,-1.25) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
		
		%B block right
		\node (15) at (1.75,-8.25) {\color{teal}$A$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}+p_B}+\rho,-b{\color{red}-p_B}+\rho)$};
		\node (4) at (-3.75,-6.75) {$({\color{red}c+p_B}+\rho+\alpha,{\color{red}-c-p_B}+\rho+\alpha)$};
		
		%A block bottom
		\node (18) at (-3,-9) {$(b{\color{red}+p_B}-f+\rho+\alpha,-b{\color{red}-p_B}+\rho)$};
		\node (19) at (-0.5,-9.5) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		{\color{olive}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.5] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);
		\path (1) edge node [left] {\tiny $S$} (24); }
		
		{\color{teal}
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);

		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{olive}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);
		\path (5) edge node [above] {\tiny $S$}  (4);}
		
		{\color{teal}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S'_{2}$ with  Update $(a,b)\mapsto (a-p_B,b+p_B)$.}
	\label{tbl:S2p}
\end{figure}




The next couple of subgames $S_3$ (\Cref{tbl:S3}), $S_4$ (\Cref{tbl:S4}) represent channel updates that were proposed by $B$, after $A$ tried to close the channel honestly and collaboratively. Similar to before, $S_3$ represents the case where $A$'s balance is increased, therefore an update from $(a,b)$  to $(a+p_A,b-p_A)$. The other subgame $S_4$ handles the case where the update increases $B$'s balance to a new state $(a-p_B,b+p_B)$.

\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{teal}$A$};
		
		%A block top
		\node (20) at (1,-2.25) {\color{olive} $B$};
		\node (2) at (1.75,-3.25) {\color{olive}$B$} ; 
		\node (3) at (-1.,-0.25) {\color{olive}$B$};
		\node (21) at (-1,0.5) {$(\alpha-\epsilon,\alpha)$};
		
		%B block left
		\node (22) at (-2.,-3.25) {$(-a,a-f+\alpha)$};
		\node (23) at (-3.5,-2.75) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
				
		%B block middle
		\node (8) at (-2.5,-2) {$(-a,-b)$};
		\node (24) at (-0.,-1.25) {$(\alpha,\alpha)$};
		\node (9) at (-1.,-2.) {$(\alpha,\alpha-\epsilon)$};
		\node (10) at (-2.25,-0.5) {\color{teal}$A$};
		
		%B block right
		\node (4) at (-2.5,-4) {$({\color{red}-p_A}+\rho+\alpha,{\color{red}p_A}+\rho+\alpha)$};
		\node (5) at (1.75,-6.75) {\color{teal}$A$};
		\node (6) at (-1,-4.5) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (7) at (1,-5.) {\color{teal}$A$};
		

		
		%A block middle
		\node (11) at (-0.75,-6.25) {$(b{\color{red}-p_A}-f+\rho+\alpha,-b{\color{red}+p_A}+\rho)$};
		\node (12) at (-2.75,-5.75) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		%A block left
		\node (13) at (-5,-0.75) {$(b-f+\alpha,-b)$};
		\node (14) at (-4.25,-1.25) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
		
		
		%A block right
		\node (15) at (1.75,-8.25) {\color{olive}$B$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}-p_A}+\rho,-b{\color{red}+p_A}+\rho)$};
		
		
		%B block bottom
		\node (18) at (-3,-9) {$(-a{\color{red}-p_A}+\rho,a{\color{red}+p_A}-f+\rho+\alpha)$};
		\node (19) at (-0.5,-9.5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		
		
		{\color{teal}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.4] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);}
		
		{\color{olive}
		\path (2) edge node [above] {\tiny $S$}  (4);
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		 
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);
		\path (3) edge node [left] {\tiny $S$} (24); 
		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{teal}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);}
		
		{\color{olive}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S_{3}$ with  Update $(a,b)\mapsto (a+p_A,b-p_A)$.}
	\label{tbl:S3}
\end{figure}


\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{teal}$A$};
		
		%A block top
		\node (20) at (1,-2.25) {\color{olive} $B$};
		\node (2) at (1.75,-3.25) {\color{olive}$B$} ; 
		\node (3) at (-1.,-0.25) {\color{olive}$B$};
		\node (21) at (-1,0.5) {$(\alpha-\epsilon,\alpha)$};
		
		%B block left
		\node (22) at (-2.,-3.25) {$(-a,a-f+\alpha)$};
		\node (23) at (-3.5,-2.75) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
				
		%B block middle
		\node (8) at (-2.5,-2) {$(-a,-b)$};
		\node (24) at (-0.,-1.25) {$(\alpha,\alpha)$};
		\node (9) at (-1.,-2.) {$(\alpha,\alpha-\epsilon)$};
		\node (10) at (-2.25,-0.5) {\color{teal}$A$};
		
		%B block right
		\node (4) at (-2.5,-4) {$({\color{red}p_B}+\rho+\alpha,{\color{red}-p_B}+\rho+\alpha)$};
		\node (5) at (1.75,-6.75) {\color{teal}$A$};
		\node (6) at (-1,-4.5) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (7) at (1,-5.) {\color{teal}$A$};
		

		
		%A block middle
		\node (11) at (-0.75,-6.25) {$(b{\color{red}+p_B}-f+\rho+\alpha,-b{\color{red}-p_B}+\rho)$};
		\node (12) at (-2.75,-5.75) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		%A block left
		\node (13) at (-5,-0.75) {$(b-f+\alpha,-b)$};
		\node (14) at (-4.25,-1.25) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
		
		
		%A block right
		\node (15) at (1.75,-8.25) {\color{olive}$B$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}+p_B}+\rho,-b{\color{red}-p_B}+\rho)$};
		
		
		%B block bottom
		\node (18) at (-3,-9) {$(-a{\color{red}+p_B}+\rho,a{\color{red}-p_B}-f+\rho+\alpha)$};
		\node (19) at (-0.5,-9.5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		
		
		{\color{teal}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.4] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);}
		
		{\color{olive}
		\path (2) edge node [above] {\tiny $S$}  (4);
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		 
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);
		\path (3) edge node [left] {\tiny $S$} (24); 
		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{teal}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);}
		
		{\color{olive}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S_{4}$ with Update $(a,b)\mapsto (a-p_B,b+p_B)$.}
	\label{tbl:S4}
\end{figure}

Finally, the subgames $S'_3$ and $S'_4$ in \Cref{tbl:S3p,tbl:S4p} handle the same situations as $S_3$ and $S_4$, except the by $A$ partially signed closing attempt is unfair and increases $A$'s outcome by $c>0$.




\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{teal}$A$};
		
		%A block top
		\node (20) at (1,-2.25) {\color{olive} $B$};
		\node (2) at (1.75,-3.25) {\color{olive}$B$} ; 
		\node (3) at (-1.,-0.25) {\color{olive}$B$};
		\node (21) at (-1,0.5) {$(\alpha-\epsilon,\alpha)$};
		
		%B block left
		\node (22) at (-2.,-3.25) {$(-a,a-f+\alpha)$};
		\node (23) at (-3.5,-2.75) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
				
		%B block middle
		\node (8) at (-3.25,-2) {$(-a,-b)$};
		\node (24) at (-0.15,-1.25) {$({\color{red}c}+\alpha,{\color{red}-c}+\alpha)$};
		\node (9) at (-1.75,-2.) {$(\alpha,\alpha-\epsilon)$};
		\node (10) at (-2.25,-0.5) {\color{teal}$A$};
		
		%B block right
		\node (4) at (-3,-4) {$({\color{red}c-p_A}+\rho+\alpha,{\color{red}-c+p_A}+\rho+\alpha)$};
		\node (5) at (1.75,-6.75) {\color{teal}$A$};
		\node (6) at (-1,-4.5) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (7) at (1,-5.) {\color{teal}$A$};
		

		
		%A block middle
		\node (11) at (-0.75,-6.25) {$(b{\color{red}-p_A}-f+\rho+\alpha,-b{\color{red}+p_A}+\rho)$};
		\node (12) at (-2.75,-5.75) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		%A block left
		\node (13) at (-5,-0.75) {$(b-f+\alpha,-b)$};
		\node (14) at (-4.35,-1.25) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
		
		
		%A block right
		\node (15) at (1.75,-8.25) {\color{olive}$B$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}-p_A}+\rho,-b{\color{red}+p_A}+\rho)$};
		
		
		%B block bottom
		\node (18) at (-3,-9) {$(-a{\color{red}-p_A}+\rho,a{\color{red}+p_A}-f+\rho+\alpha)$};
		\node (19) at (-0.5,-9.5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		
		
		{\color{teal}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.4] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);}
		
		{\color{olive}
		\path (2) edge node [above] {\tiny $S$}  (4);
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		 
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);
		\path (3) edge node [left] {\tiny $S$} (24); 
		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{teal}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);}
		
		{\color{olive}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S'_{3}$ with Update $(a,b)\mapsto (a+p_A,b-p_A)$.}
	\label{tbl:S3p}
\end{figure}



\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',auto,node distance=2cm, el/.style = {inner sep=2pt, align=left, sloped}]
		\node (1) at (1.75,0.75) {\color{teal}$A$};
		
		%A block top
		\node (20) at (1,-2.25) {\color{olive} $B$};
		\node (2) at (1.75,-3.25) {\color{olive}$B$} ; 
		\node (3) at (-1.,-0.25) {\color{olive}$B$};
		\node (21) at (-1,0.5) {$(\alpha-\epsilon,\alpha)$};
		
		%B block left
		\node (22) at (-2.,-3.25) {$(-a,a-f+\alpha)$};
		\node (23) at (-3.5,-2.75) {$(d_A+\alpha-\epsilon,-d_A+\alpha)$};
				
		%B block middle
		\node (8) at (-3.25,-2) {$(-a,-b)$};
		\node (24) at (-0.15,-1.25) {$({\color{red}c}+\alpha,{\color{red}-c}+\alpha)$};
		\node (9) at (-1.75,-2.) {$(\alpha,\alpha-\epsilon)$};
		\node (10) at (-2.25,-0.5) {\color{teal}$A$};
		
		%B block right
		\node (4) at (-3,-4) {$({\color{red}c+p_B}+\rho+\alpha,{\color{red}-c-p_B}+\rho+\alpha)$};
		\node (5) at (1.75,-6.75) {\color{teal}$A$};
		\node (6) at (-1,-4.5) {$(\rho+\alpha,\rho+\alpha-\epsilon)$};
		\node (7) at (1,-5.) {\color{teal}$A$};
		

		
		%A block middle
		\node (11) at (-0.75,-6.25) {$(b{\color{red}+p_B}-f+\rho+\alpha,-b{\color{red}-p_B}+\rho)$};
		\node (12) at (-2.75,-5.75) {$(-d_B+\rho+\alpha,d_B+\rho+\alpha-\epsilon)$};
		
		%A block left
		\node (13) at (-5,-0.75) {$(b-f+\alpha,-b)$};
		\node (14) at (-4.35,-1.25) {$(-d_B+\alpha,d_B+\alpha-\epsilon)$};
		
		
		%A block right
		\node (15) at (1.75,-8.25) {\color{olive}$B$};
		\node (16) at (-0.5,-8) {$(\rho+\alpha-\epsilon,\rho+\alpha)$};
		\node (17) at (-2.5,-7.5) {$(-a{\color{red}+p_B}+\rho,-b{\color{red}-p_B}+\rho)$};
		
		
		%B block bottom
		\node (18) at (-3,-9) {$(-a{\color{red}+p_B}+\rho,a{\color{red}-p_B}-f+\rho+\alpha)$};
		\node (19) at (-0.5,-9.5) {$(d_A+\rho+\alpha-\epsilon,-d_A+\rho+\alpha)$};
		
		
		
		{\color{teal}
		\path (1) edge node [left, pos=0.5] {\tiny $A$}  (2);
		\path (1) edge node [above, pos=0.4] {\tiny $I$}  (3); 
		\path (1) edge node [left]  {\tiny $D$} (20);
		\path (1) edge node [above]  {\tiny $H$} (21);}
		
		{\color{olive}
		\path (2) edge node [above] {\tiny $S$}  (4);
		\path (2) edge node [left, pos=0.3] {\tiny $I$}  (5);
		\path (2) edge node [above] {\tiny $H$}  (6);
		\path (2) edge node [left] {\tiny $D$}  (7);
		 
		\path (3) edge node [above, pos=0.5] {\tiny $I$}  (8);
		\path (3) edge node [left] {\tiny $S$} (24); 
		\path (3) edge node [left] {\tiny $H$}  (9);
		\path (3) edge node [above] {\tiny $D$}  (10); 
		
		\path (20) edge node [below] {\tiny $I$} (23); 
		\path (20) edge node [below] {\tiny $P$} (22);}
		
		{\color{teal}
		\path (7) edge node [below] {\tiny $P$}  (11); 
		\path (7) edge node [below] {\tiny $I$}  (12);
		
		\path (10) edge node [above, pos=0.7] {\tiny $P$}  (13);
		\path (10) edge node [below] {\tiny $I$}  (14);
		
		\path (5) edge node [left] {\tiny $D$}  (15);
		\path (5) edge node [above] {\tiny $H$}  (16); 
		\path (5) edge node [above] {\tiny $I$}  (17);}
		
		{\color{olive}
		\path (15) edge node [below] {\tiny $P$}  (18);
		\path (15) edge node [below] {\tiny $I$}  (19);}
	\end{tikzpicture}
	\caption{Subgame $S'_{4}$ with Update $(a,b)\mapsto (a-p_B,b+p_B)$.}
	\label{tbl:S4p}
\end{figure}


==> includes/authors.tex <==
\author{%
Sophie~Rain\inst{1}\orcidID{0000-0002-8940-4989},
Zeta Avarikioti\inst{2},
Laura Kov\'acs\inst{1}\orcidID{0000-0003-0845-5811},
Matteo Maffei\inst{1}
}
\institute{%
	TU Wien,~Austria
	\and
	IST Austria
}


==> includes/defs.tex <==
% BBL underfull fixes
\apptocmd{\thebibliography}{\raggedright}{}{}

% ERC-20 datatypes
\newcommand{\bool}{\texttt{boolean}}
\newcommand{\addr}{\texttt{address}}
\newcommand{\uint}{\texttt{uint}}

% Tables
\captionsetup[table]{name=Table}

% Listings
\definecolor{mycomment}{rgb}{0.05,0.35,0.05}
\definecolor{mykeyword}{HTML}{4c1b54}
\definecolor{lightgreen}{HTML}{d9ead3}
\definecolor{lightblue}{HTML}{cfe2f3}
\definecolor{lightpink}{HTML}{ead1dc}
\definecolor{lightyellow}{HTML}{fff2cc}

\lstset{
	basicstyle=\small\ttfamily,
	commentstyle=\color{mycomment},
	keywordstyle=\bfseries\color{mykeyword},
	breaklines=true,
	frame=bottomline,
	escapechar=@,
	tabsize=4,
	language=Python,,
	language=Python,
	morekeywords={assert,each},
	frame=single,
	emph={Address,Nat,mint},
	emphstyle=\bfseries,
	emph={[2]balance},
	emphstyle={[2]\underbar}
}

\newcommand{\listingrule}{\noindent\rule{\columnwidth}{0.2pt}}

\newcommand{\define}{\triangleq}

% Sum logic
\newcommand{\SL}{{\textsc{SL}}}
\newcommand{\PA}{{\textsc{PA}}}
\newcommand{\srt}{\mbox{{\tt sort}}}
\newcommand{\Lang}{\mathcal{L}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcC}{\mathcal{C}}


\newcommand{\Nat}{\textnormal{\texttt{Nat}}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\domain}{\mathcal{D}}
\newcommand{\interp}{\mathcal{I}}
\newcommand{\structure}[1]{\text{STRUCT}\brackets{#1}}

\newcommand{\sat}{\vDash}
\newcommand{\nsat}{\nvDash}
\newcommand{\To}{\Rightarrow}

\newcommand{\bigland}{\bigwedge}
\newcommand{\biglor}{\bigvee}

\newcommand{\argmax}{\mathop{\arg\max}}
\newcommand{\argmin}{\mathop{\arg\min}}

\newcommand{\dosub}[2]{#2 / #1}

\NewDocumentCommand{\sub}{O{x}O{\alpha}}{
	\brackets{ \dosub{#1}{#2} }%
}

\NewDocumentCommand{\subs}{O{}O{r}O{x}O{\alpha}O{}}{%
	\brackets{ #1 \dosub{#3_1}{#4_1}, \dots, \dosub{#3_{#2}}{#4_{#2}} #5 }
}

\NewDocumentCommand{\subsi}{O{}O{r}O{x}O{\alpha}O{}}{%
	\brackets{ #1 \dosub{#3_1}{#4_{i_1}}, \dots, \dosub{#3_{#2}}{#4_{i_{#2}}} #5 }
}

\newcommand{\ifelsedef}[3]
{
	\left\{
	\begin{array}{ll}
		#1 & \mbox{if } #2 \\
		#3 & \mbox{otherwise}
	\end{array}
	\right.
}

\newcommand{\sort}[1]{\boldsymbol{#1}}
\newcommand{\mS}{\mathcal{S}}

\Crefname{formula}{Formula}{Formulas}
\Crefname{nclaim}{Claim}{Claims}
\Crefname{cong}{Congruence Condition}{Congruence Conditions}

% Environments
\spnewtheorem{observation}{Observation}{\itshape}{\rmfamily}
\spnewtheorem{nclaim}{Claim}{\itshape}{\rmfamily}



% Proof environments
\makeatletter
\NewDocumentEnvironment{longproof}{m}
{%
	\setcounter{proofpart}{0}%
	\setcounter{proofstep}{0}%
	\setcounter{proofcase}{0}%
	\noindent\underline{\textbf{\textit{Proof of} {#1}}}%
	\par\nobreak\smallskip%
	\@afterheading
}
{\begin{center}\textit{Q.E.D.} {#1}.\end{center}}
\makeatother

\makeatletter
\newcounter{proofpart}
\newcommand{\proofpart}[1]{%
	\stepcounter{proofpart}%
	\noindent\textbf{Part \theproofpart: #1}\par\nobreak\smallskip
	\setcounter{proofstep}{0}
	\setcounter{proofcase}{0}
	\@afterheading
}
\makeatother

\makeatletter
\newcounter{proofstep}
\newcommand{\proofstep}[1]{%
	\par
	\stepcounter{proofstep}%
	\noindent\underline{Step 
		\ifnum0<\value{proofpart}%
		\theproofpart.%
		\fi
		\theproofstep}: #1\par\nobreak\smallskip
	\setcounter{proofcase}{0}
}
\makeatother

\makeatletter
\newcounter{proofcase}
\newcommand{\proofcase}[1]{%
	\par
	\stepcounter{proofcase}%
	\noindent\textit{Case 
		\ifnum0<\value{proofpart}%
		\theproofpart.%
		\fi
		\ifnum0<\value{proofstep}%
		\theproofstep.%
		\fi
		\theproofcase}: #1\par\nobreak\smallskip
}
\makeatother

%shortcuts encodings
\newcommand{\atexttt}[1]{\textnormal{\texttt{#1}}}

\newcommand{\isactive}{\textbf{active}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\I}{\mathbb{I}}

\newcommand{\bank}{\textbf{bank}}
\newcommand{\total}{\atexttt{total}}

\newcommand{\Coin}{\atexttt{Coin}}
\newcommand{\Addr}{\atexttt{Address}}

\newcommand{\ite}{\text{if-then-else}}
\newcommand{\mC}{\mathcal{C}}

\newcommand{\ac}{\atexttt{active}}
\newcommand{\hc}{\atexttt{has-coin}}

\newcommand{\mA}{\mathcal{A}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\proofend}{	\begin{flushright} $\square$ \end{flushright}}
\newcommand{\bal}{\atexttt{bal}}

\newcommand{\parens}[1] { \left( #1 \right)}
\newcommand{\pair}[2]{\parens{#1,#2}}
\newcommand{\braces}[1]{ \left\{ #1 \right\} }
\newcommand{\brackets}[1]{ \left[ #1 \right] }
\newcommand{\abs}[1]{
	\left|#1\right|
}

\newcommand{\N}{\mathbb{N}}
\newcommand{\liff}{\leftrightarrow}
\newcommand{\ind}{\atexttt{idx}}
\newcommand{\inv}{\atexttt{inv}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\old}{\atexttt{old-}}
\newcommand{\new}{\atexttt{new-}}

\newcommand{\world}{\atexttt{world}}

\newcommand{\oldworld}{\old\world}
\newcommand{\newworld}{\new\world}

\newcommand{\mint}{\atexttt{mint}}
\newcommand{\transfer}{\atexttt{transferFrom}}

\newcommand{\msum}{\atexttt{sum}}
\newcommand{\oldsum}{\old\msum}
\newcommand{\newsum}{\new\msum}
\newcommand{\oldbal}{\old\bal}
\newcommand{\newbal}{\new\bal}
\newcommand{\mcount}{\atexttt{count}}
\newcommand{\ocount}{\old\mcount}
\newcommand{\ncount}{\new\mcount}
\newcommand{\oind}{\old\ind}
\newcommand{\nind}{\new\ind}

\newcommand{\zbal}{\atexttt{z-bal}}
\newcommand{\zhc}{\atexttt{z-has-coin}}
\newcommand{\zact}{\atexttt{z-active}}
\newcommand{\zsum}{\atexttt{z-sum}}
\newcommand{\zcount}{\atexttt{z-count}}
\newcommand{\zind}{\atexttt{z-idx}}

\newcommand{\xhascoin}{\atexttt{x-has-coin}}
\newcommand{\xsum}{\atexttt{x-sum}}
\newcommand{\xcount}{\atexttt{x-count}}
\newcommand{\xind}{\atexttt{x-idx}}
\newcommand{\xbal}{\atexttt{x-bal}}
\newcommand{\xactive}{\atexttt{x-active}}

\newcommand{\ybal}{\atexttt{y-bal}}
\newcommand{\yhascoin}{\atexttt{y-has-coin}}
\newcommand{\yactive}{\atexttt{y-active}}
\newcommand{\ysum}{\atexttt{y-sum}}

\newcommand{\oldhc}{\old\hc}
\newcommand{\newhc}{\new\hc}
\newcommand{\oldact}{\old\ac}
\newcommand{\newact}{\new\ac}

\newcommand{\suma}{\sum_{a \in \Addr}}
\newcommand{\aco}{\ac_{\,\atexttt{1}}}
\newcommand{\act}{\ac_{\,\atexttt{2}}}
\newcommand{\hco}{\hc_{\,\atexttt{1}}}
\newcommand{\hct}{\hc_{\,\atexttt{2}}}

\newcommand{\ufenc}{\atexttt{uf}}
\newcommand{\intenc}{\atexttt{int}}
\newcommand{\natenc}{\atexttt{nat}}
\newcommand{\idenc}{\atexttt{id}}

\newcommand{\twocm}{two-counter machine}
\newcommand{\Twocm}{Two-counter machine}
\newcommand{\TwoCM}{Two-Counter Machine}
\newcommand{\twocms}{two-counter machines}
\newcommand{\pc}{\textsc{pc}}

==> includes/references.tex <==





% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)

%\bibliographystyle{IEEEtran}
\bibliography{includes/references}


==> includes/related.tex <==
\section{Related work}
Our work is mainly based on the results of \cite{CITE}. 
The game-theoretic models presented in \cite{CITE} provide a good basis, however they are not yet sufficient. 
We extended the closing game drastically, by aligning the utilities to the monetary outcome, considering random deviation from the protocol including dishonest closing attempts and incorporating fees for revocation transactions. 
Further, we proved their routing game insufficient, by refining it in such a way that it can capture the Wormhole attack, which Lightning's routing is vulnerable to. 
Moreover, we propose an adaption of the security properties introduced in \cite{CITE}.\\





Mention:\\
Awareness and other things about NE \cite{HalpernNE} \textcolor{orange}{More details needed.}\\


Related Work:\\
\paragraph{Other work on game-theory in the blockchain domain}

 Games for Mining \cite{MiningGames}.\\
Games for Payment Channel Network creation \cite{RideTheLightning}.\\
Distributed computing meets game theory \cite{DCMeetsGameTheory} (intro of k-resilient NE, t-immunity, show k-resilient NE exist for secret sharing and multiparty computation).\\
Games for Smart Contracts \cite{QuantAnalysisSC} introducing simplified language to formally capture smart contracts and automatically translate it to a concurrent game (game with states), framework for quantitative analysis of contracts, \textcolor{orange}{emphasize difference to us, do different kind of analysis? not rigorously but using suspicious results?.}\\
Game-theory to provide Secure pseudo-random number generation for smart contracts \cite{ProbSC}.\\


\paragraph{Other formal verification approaches for security in distributed computing}

\cite{DiffApp1}
\cite{AdDiffApp1}
\cite{DiffApp2}
\cite{SurveyOnBC}
\cite{OverviewOffChain}
\cite{SecAnalysis}\\

Work on Off-Chain Channels:\\
\cite{GenChannels}
\cite{Brick}
\cite{SecEffChannels}{ \color{orange}
Many talk about incentive compatibility, no one has a proper model/proof.\\
}
